Efficient Adaptation of Reinforcement Learning Agents to Sudden Environmental Change

Real-world autonomous decision-making systems, from robots to recommendation engines, must operate in environments that change over time. While deep reinforcement learning (RL) has shown an impressive ability to learn optimal policies in stationary environments, most methods are data intensive and assume a world that does not change between training and test time. As a result, conventional RL methods struggle to adapt when conditions change. This poses a fundamental challenge: how can RL agents efficiently adapt their behavior when encountering novel environmental changes during deployment without catastrophically forgetting useful prior knowledge? This dissertation demonstrates that efficient online adaptation requires two key capabilities: (1) prioritized exploration and sampling strategies that help identify and learn from relevant experiences, and (2) selective preservation of prior knowledge through structured representations that can be updated without disruption to reusable components.

==> archive/7a_pretraining_chapt.tex <==
\chapter{Pre-training and Offline-to-Online Partial Transfer of World Models}
\label{chapt:pretraining}

Model-based reinforcement learning has long been thought to be critical to efficient adaptation of reinforcement learning agents~\cite{precup1997multi,daw2011model,khetarpal2022towards}. 
In theory, a model of the world's dynamics provides agents the ability to plan and learn directly from the world model. 
When these world models are trained on a large and diverse enough body of data, agents with world models can react to environment changes rapidly without requiring the agent to repeatedly interact with novel, potentially dangerous phenomena. 

Despite this, most modern model-based deep reinforcement learning methods are designed to learn to execute a task from a \textit{tabula rasa}~\cite{agarwal2022beyond} state, meaning that the agent initialized for interactive training with random weights. 
In fact, most work that studies learning sequential decision models, both with RL and alternative techniques like imitation learning, is studied in the context of learning to solve problems from randomly initialized parameters~\cite{wang2022drlsurvey,lazaridis2020deep}. 
While historically RL models have been trained from randomly initialized parameters, in the context of modern deep learning with large neural networks~\cite{erhan2010pretraining,devlin2019bert}, pre-training a model is widely accepted as critical to maximizing down stream task performance, robustness~\cite{hendrycks2019using}, and adaptability of a model~\cite{kim2022broad,gururangan2020don}. 

In this dissertation, our focus on the adaptability of sequential decision making models means a model's prior knowledge is of the utmost importance.  
In addition, the study of knowledge preservation in transfer is both more difficult
\MarkLeft{than what?} 
and applies to a smaller body of environments when the knowledge is attained in the context of tabula rasa training. 
\julia{I think I know what you mean but a little confusing - come back to this}
To better understand the effect of pre-training on adaptation and knowledge transfer, I examine diverse offline decision making data used to pre-train the model-based DreamerV3 reinforcement learning agent. 
Specifically, in the Robosuite robot manipulation environment using the demonstration data collected in the LIBERO dataset, I explore the impact of different pre-training and data augmentation techniques and training processes on both pre-training and fine tuning performance and the transfer of parts of the pre-trained modeld. 
To our knowledge, this represents the first attempt to train Dreamer offline on demonstration data, without additional models or learning techniques like inverse models or behavior cloning policies, for the purposes of adaptability and knowledge preservation. 
While the findings described in this chapter are only studied in the Robosuite manipulation setting, the findings are likely applicable broadly as DreamerV3 is designed and tuned to, in the words of the original authors, "master a wide range of applications with fixed hyperparameters."
\julia{there's a logical leap here that I'm missing}

In Section~\ref{sec:pretraining:related} I provide a brief overview of the prior work specific to pre-training and partial model training. 
Following that, in Section~\ref{sec:pretraining:theory} I return to the algorithmic formulation of Dreamer and highlight the challenges that exist in pre-training this specific online model-based reinforcement learning method. 
In Section~\ref{sec:pretraining:experiments} I describe the details of experimental setup with the questions that motivate the different experiments, and provide the results of those experiments. 
Finally, I discuss what the results of the experiments tell us about the efficacy of pre-training Dreamer offline for adaptation and knowledge preservation. 
At a high level, we found that the diversity of the pre-training dataset was critical for fine tuning and that naive fine tuning of all of the pre-trained weights results in a weaker model than transferring parts of the pre-trained models. 
Moreover, we demonstrate using the Concept Bottleneck World Model variant of Dreamer---detailed in Chapter~\ref{chapt:cbwm}---that knowledge preservation and its impact on adaptation efficiency is sensitive to pre-training methods.

\section{Related Work}
\label{sec:pretraining:related}

The ability of deep neural networks to scale learning performance with data is one of the reasons why pre-training with non-task data is so effective~\cite{erhan2010pretraining}. 
Motivated by the widespread interest in using deep reinforcement learning for agents learning from visual observations, the most straightforward way to improve agent performance using offline data is to pre-train only the observation encoder~\cite{stooke2021decoupling,parisi2022pretrain}. 
While pre-training the visual encoder avoids many of the challenges and complexities of sequential decision making, the impact on agent performance is unreliable~\cite{shah2021rrl}. 

Offline pre-training reinforcement learning agent behavior can be largely divided into three types of approaches: imitation learning, task-agnostic exploration, or offline reinforcement learning. 
Imitation learning-based pre-training, using techniques like behavior cloning to establish a baseline policy, is often used to improve the sample efficiency of learning policies for complex problem spaces, such as the manipulation of arbitrary objects~\cite{kalashnikov2018scalable}. 
As a result, accumulating datasets of internet-scale demonstrations with different tasks shows great promise for GPT-like policy foundation models~\cite{openxembodiment2024}.
Video Pre-Training (VPT)~\cite{baker2022video} demonstrates that an inverse control-prediction model trained on a small set of demonstrations can be used to supervise imitation learning on a significantly larger dataset of action-free sequence data.
Imitation learning-based pre-training, however, makes the assumption that the state action space is sufficiently smooth such that expert demonstrations cover all situations an agent will encounter, which is not always true. 

Task agnostic exploration assumes a phase during which the reinforcement learning agent is not necessarily given access to the task on which it will be evaluated, but is given access to the environment for interaction. 
Also referred to in off-policy reinforcement learning as ``warm starting,'' unsupervised exploration pre-training usually attempts to cover the state-action space by exploring the space by maximizing surrogate objectives~\cite{andrychowicz2017hindsight,liu2021apt} 
(for a more detailed overview of exploration techniques see Chapters~\ref{chapt:background} and~\ref{chapt:transx}).
The most prominent examples of this employed in pre-training Dreamer are Plan2Explore~\cite{sekar2020planning} in which the policy maximizes uncertainty as the reward, and LEXA~\cite{mendonca2021lexa} which (provided a pre-trained world model) trains an exploration policy that learns to reach novel states. 
However, pre-training with task-agnostic exploration rarely reduces the total amount of environment interaction needed to learn a policy, and as such does not overall improve the interactive sample efficiency of reinforcement learning agents.
Moreover, if the environment is available for pre-training, there are many situations in which environment access is limited or too slow and difficult for interactive pre-training.

For offline reinforcement learning-based pre-training, offline model-free reinforcement learning has seen more research interest than model based methods. 
Two popular methods that address issues inherent in offline algorithms for fine tuning are Conservative Q-Learning (CQL)~\cite{kumar2020cql}, which addresses the distributional shift that occurs when an offline policy encounters novel states during online adaptation, and Batch-Constrained Q-learning (BCQ)~\cite{fujimoto2019bcq}, which constrains the policy in online training to actions close to those in the offline dataset. 
Fewer efforts have been made to formulate offline model-based reinforcement learning approaches~\cite{he2023surveyofflinemodelbasedreinforcement}. 
Notably, Model-Based Offline Reinforcement Learning (MOReL)~\cite{kidambi2020morel} learns a pessimistic MDP to provide lower-bound performance guarantees. 
Although all these approaches are theoretically sound, in practice they can be overly conservative and use suboptimal heuristics and hyperparameters~\cite{lu2022revisiting}, limiting performance on some tasks, especially when fine tuned. 
% and there is evidence that good offline rl performance does not mean good online training performance

Fine tuning offline pre-trained RL agents is sufficiently challenging~\cite{lee2022offline,wolczyk24finetuning} that a recent body of work has focused on improving the two-step process of ``offline-to-online reinforcement learning.'' 
The difficulties that arise during the offline-to-online conversion are usually attributed to the sudden shift from the offline state-action distribution to the online state-action distribution (which can lead to bootstrapping errors in fine tuning), overfitting to on-policy demonstrations leading to problems reasoning over off-policy dynamics, and the impact of non-stationarity of rewards on the training of the value function~\cite{levine2020offline}.
One of the first efforts in offline-to-online RL is Advantage-Weighted Actor Critic (AWAC)~\cite{nair2021awac}, which effectively separates learning into supervised learning of the policy and reinforcement learning of the critic to mitigate the negative effects of shifting from the offline data distribution to the online data distribution.
Building off of the work by AWAC, methods reduce the impact of the offline-to-online distribution shift by adding uncertainty to reduce policy exploitation~\cite{rafailov23moto}, smoothing the transition using a blend of offline and online data~\cite{lee2022offline,mao2022moore}, and by adding constraints such as behavior cloning losses~\cite{wang2024o2ac} that can be gradually reduced over training. 


There have been a small number of attempts to reformulate model-based RL methods like Dreamer to work both offline and online. 
The simplest method of doing this is to follow the training process of Ha and Schmidhuber~\cite{ha2018recurrent}, where instead of training Dreamer in an ``interleaved'' fashion as designed, where for every step the agent takes in the environment the world model \textit{and} the agent are updated, the agent is trained in ``phases.'' First, the world model is trained on interaction data, and then the world model is frozen and behavior training phase begins~\cite{lu2023challenges, wang2024making}. 
By splitting the training into phases, each phase can be executed offline. 
However, as highlighted by prior work on exploration for Dreamer agents~\cite{sekar2020planning,mendonca2021lexa}, the phase-based approach only works for tasks where exploration is trivial or unimportant. 
Moreover, this makes the assumption that the world model does not require the agent learning process to learn the task effectively, which is in some ways the assumption of imitation learning-based pre-training, but applied to an ``expert'' world model instead of policy. 
One work that pre-trains Dreamer using interaction data in the intended interleaved fashion is the APV method~\cite{seo2022pretraining}, which still modifies the process with an additional module to learn ``action-free'' models before fine tuning online.  
As of this writing, there has been no prior work focused on how to effectively pre-train an unmodified Dreamer agent using end-to-end interleaved training process using both offline and online interaction data. 



\section{Challenges in Interleaved Pre-training of World Model Agents}
\label{sec:pretraining:theory} 

Revisiting the discussion from Chapter~\ref{chapt:background}, the combination of characteristics that most distinguishes the Dreamer~\cite{hafner2019dream} family of model-based reinforcement learning (MBRL) algorithms from other MBRL algorithms is:
\begin{enumerate}
    \item The RSSM world model architecture (Equation~\ref{eq:dreamer:wm}) that models the transition function as a recurrent variational state space,
    \item The use of observation reconstruction as a primary loss in learning the world model,
    \item The formulation of the behavior policy as a latent actor-critic learning only from rollouts in the world model latent space,
    \item Learning both the actor-critic and world model in an interleaved fashion as opposed to in separate phases. 
\end{enumerate}

Maintaining all of these characteristics for both pre-training and fine tuning is challenging and begs the question: ``Why \textit{not} use other methods?'' 
An effort is made to preserve this formulation because recent work postulates that the Dreamer formulation models adaptable human cognition more closely than other approaches~\cite{pearson2019human,mattar2022planning,kudithipudi2022biological,deperrois2024learning}.
Moreover, with the ability of the actor-critic to be trained solely in the ``imagination'' of the world model, Dreamer is well-suited to solving the problem of learning without interacting.
Provided a reasonable approximation of the true reward model and good coverage of the state-actions space, behavior learning theoretically does not require any environment interaction as the actor-critic learns entirely in the world model's embedding space.
\MarkRight{Doesn't this cut against your argument about why to use dreamer instead of other models?}
\jb{yeah the phraseing is wrong, I'll fix it when we try to publish}
Lastly, the Dreamer architecture is difficult to train piece-wise because the input to the policy is an embedded state, and the world model learning depends on agent behavior to explore so as to avoid overfitting the world model to only the dynamics of the optimal path. 



\subsection{Impact of Partial Model Transfer on Interleaved Actor-Critic}

One of the primary concerns with transferring a pre-trained world model agent is the cascading impact of partial transfers on the actor-critic.
Consider the problem of transferring solely the  world model and not the actor or critic models. 
This is a reasonable approach as prior work in offline-to-online RL caution against transferring overfit actors and critics with poor bootstrapping ability~\cite{wang2024o2ac}, and model-based exploration pre-training works do not transfer the exploration policy when fine tuning~\cite{sekar2020planning,mendonca2021lexa}.  
In actor-critic training, the data used to train the critic is drawn from initial embeddings of real-world states, followed by imagined latent states as generated by the transition predictor, all valued by the rewards from the reward predictor. 
The Dreamer algorithm assumes \textit{tabula rasa} learning, so the distribution of latent states sampled by a random policy $p_{\pi_U}(s)$, with random embeddings and rewards from the initial transition and reward predictors. 
This gives a noisy $\lambda$-error calculation (Equation~\ref{eq:dreamer:tdlambda}), which will produce high gradients that accurately reflect the need for the critic to make large changes to its parameters 

However, assuming instead that the transition and reward prediction models are trained on expert demonstrations, a different outcome emerges. 
When trained transition and reward prediction models are used in policy learning, these models will predict that latent data distributed according to random actions $p_{\pi_U}(s)$ are relatively close in latent space and all have rewards near zero. 
As a result, the critic will predict similar values for all states, leading to a low $\lambda$-error. 
The gradients for much of the early online learning period will be inaccurately small, leading to slower behavior learning than in tabula rasa learning.

\begin{theorem}
Let actor $\pi_{\theta}$ and critic $v_{\psi}$ be randomly initialized models such that their outputs are distributed as $U(s_t)$. If transition predictor $g_\phi^*$ and reward predictor $\mathcal{R}_\phi^*$ are optimized to predict the online task dynamics, then for small $\epsilon$, $\mathcal{L}_0(\psi) - \varepsilon = 0$ and $\mathcal{L}_0(\theta \mid \phi^*) < \mathcal{L}_0(\theta \mid \phi^*)$.
\end{theorem}
\begin{proof}

Let $o_t \sim p_{U}(s)$ be the set of initial observations distributed according to the sequential actions of a random actor and let the embeddings $\{s_1\} e_\phi(o_t)$ serve as initial states.
Batched horizon $H$ length trajectories of states, actions, and rewards,  
$\{s,a,r,s^{\prime}\}_\tau \in B(\theta,\phi), \tau=[t:t+H]$ 
are generated according to learnable models $\pi_{\theta}$, $g_\phi$, and $\mathcal{R}_\phi$.
For \textit{tabula rasa} learning---where by initialization $\pi_{\theta}$ and $g_\phi$ are distributed uniformly in $[-1,1]$, the critic $v_{\psi}$ is a deterministic random projection, and $\mathcal{R}_\phi$ is distributed as a univariate Gaussian with unit variance and $\mu=0.1$---call the data generated by these models $B^0$.
For pre-trained learning---where $g_\phi^*$ and $\mathcal{R}_\phi^*$ are similarly distributed but with optimized parameters---call the data generated by these models $B^{\phi^*}$.

% \Mark{what is going on with formatting here? Is this a subsection or a continuation of the proof?}
% \jb{continuation of the proof. ill just drop the 'critic' heading when i move it to the appendix}

Expanding the terms of the recursion over Equation~\ref{eq:dreamer:tdlambda} and sum from Equation~\ref{eq:dreamer:critic_loss} using the definition of the expected $\lambda$-return, we have: 

\begin{align*}
    V_t^\lambda =& r_t + \hat{\gamma}_t \left((1-\lambda) v_\psi\left(s_{t+1}\right)
    +\lambda V_{t+1}^\lambda\right) \\
    V_{t=H-1}^\lambda =& r_{H-1} + \hat{\gamma}_{H-1} v_{\psi}(s_H)\\
    V_{t=H-2}^\lambda =& r_{H-2} + \hat{\gamma}_{H-2} \left( 
    % (1-\lambda) \sum_{\tau \geq H-1}^{H} (\hat{\gamma}^{\tau-H-1} \hat{r}_\tau) 
    (1-\lambda) v_{\psi}(s_{H-1}) 
    + \lambda V_{H-1}^\lambda  
    \right) \\
    & ...  \\
    V_{t=2}^\lambda =& r_{2} + \hat{\gamma}_{2} \left( 
    (1-\lambda) v_{\psi}(s_{3}) 
    + \lambda V_{3}^\lambda  
    \right) \\
    V_{t=1}^\lambda =& r_{1} + \hat{\gamma}_{1} \left( 
    (1-\lambda) v_{\psi}(s_{2}) 
    + \lambda V_{2}^\lambda  
    \right) \\
    % V_{t=1}^\lambda =& r_1 + \hat{\gamma}_1 \left( 
    % (1-\lambda) \sum_{\tau \geq 2}^{H} (\hat{\gamma}^{\tau-2} \hat{r}_\tau) 
    % + \lambda V_{2}^\lambda  
    % \right) \\
    %  & ... +& \lambda \hat{\gamma}^{H} \hat{r}_H \right) \\ 
    % \epsilon^\lambda =& v_{\psi}(s_t) - \operatorname{sg}\left(V_t^\lambda\right)
\end{align*}

\noindent First considering $B^0$, given this weighted average---exponential in horizon length---when the  states $s_t$ are distributed uniform randomly the critic as a random projection of that state will result in a diverse set of values $v_{\psi}(s_t)$. Combined with $r_t$ as a stochastic random projection, in the calculation of $\lambda$-error, $v_{\psi}(s_t)$ and $V_t^\lambda$ are not close for any given $t$ leading to high loss. 
On the other hand, if $v_{\psi}(s_H)$ is well-trained, regardless of reward function, $v_{\psi}(s_t)$ and $V_t^\lambda$ will be close, so $\lambda$-error and loss will be low.

However, when considering $B^{\phi^*}$, the states $s_t$ are concentrated as due to the trained transition predictor. 
This is because---especially in continuous control---random actions through a smooth space such as that of the learned transition predictor constitutes a generic random walk, and with distributed actors diffuse Brownian motion. 
As such, given highly similar initial states and a fixed time horizon, in the limit of initial sample size and number of distributed actors the distribution of visited states will follow a compact normal distribution with $\mu=0$ in the transition predictor's embedding space~\cite{arfken2011mathematical} following the equation for the density of particles emanating from a single point:
\begin{equation*}
    p(s_t)_\pi \propto \frac{N}{\sqrt{4\pi H}} \exp\left(-\frac{x^2}{4H}\right)
\end{equation*}
\noindent where, assuming constant diffusivity, $N$ is the number of ``random walks,'' which in our case is a function of number of actors and number of initial states, and $H$ is the horizon.
As our policy has an entropy maximization term and therefore forms a maximal entropy random walk~\cite{duda2012maximal}, this normal assumption forms an upper bound on state distribution density and is a reasonable approximation for small values of $H$.

In addition, $B^{\phi^*}$ has a trained reward function. Even with a dense reward, but especially a with a sparse reward, task design is such that states near the initial position typically have zero reward. 
Returning then to our TD($\lambda$) equations, to consider how the error term changes for a random or optimized critic, we can see that with all of the reward terms near zero, all $\lambda$-error terms for all $t$ become random projections centered on zero, making them zero in expectation. 
When the critic is not randomly initialized, the same phenomenon occurs but with less standard deviation. 
As a result, value loss tends to zero regardless of critic accuracy. 
% , and the value terms, as a random projection of a $\mu=0$ normal distribution is also 

% \begin{align*}
%     V_{t=H-1}^\lambda =&  \hat{\gamma}_{H-1} v_{\psi}(s_H) \\
%     V_{t=H-2}^\lambda =&  \hat{\gamma}_{H-2} v_{\psi}(s_{H-1}) - \hat{\gamma}_{H-2} \lambda v_{\psi}(s_{H-1}) + \hat{\gamma}_{H-2} \hat{\gamma}_{H-1} \lambda v_{\psi}(s_H)\\
%     V_{t=H-3}^\lambda =&  \hat{\gamma}_{H-3} (1-\lambda) v_{\psi}(s_{H-2}) + \hat{\gamma}_{H-3} \lambda \hat{\gamma}_{H-2} v_{\psi}(s_{H-1}) - \lambda \hat{\gamma}_{H-2} \lambda) v_{\psi}(s_{H-1}) + \lambda \hat{\gamma}_{H-2} \hat{\gamma}_{H-1} \lambda v_{\psi}(s_H) \\
%     & ...  \\
%     V_{t}^\lambda =& \sum^H_{t=1} \hat{\gamma}_{H-2} (1-\lambda) v_{\psi}(s_H-1) + \hat{\gamma}_{H-2} \hat{\gamma}_{H-1} \lambda v_{\psi}(s_H) \\
%     % V_{t=1}^\lambda =& r_1 + \hat{\gamma}_1 \left( 
%     % (1-\lambda) \sum_{\tau \geq 2}^{H} (\hat{\gamma}^{\tau-2} \hat{r}_\tau) 
%     % + \lambda V_{2}^\lambda  
%     % \right) \\
%     %  & ... +& \lambda \hat{\gamma}^{H} \hat{r}_H \right) \\ 
%     % \epsilon^\lambda =& v_{\psi}(s_t) - \operatorname{sg}\left(V_t^\lambda\right)
% \end{align*}

% Fun
\end{proof}

\subsection{Transfer Learning and Partial Model Adaptation}
Motivated by this interleaved critic learning issue and the typical issues of distribution shift associated with offline-to-online learning, we conducted systematic experiments on the transferability of various pre-trained weights and submodules from within our world model architecture. 
This is similar to partial model learning in reinforcement learning \cite{precup1997multi,talvitie2008local,khetarpal2021partial,alver2024partial}, where dynamics models are specialized to predict behaviors within localized regions of the state-action space. 
Instead of learning a model specific to a subspace, the experiments in this work reveal the submodules of world model agents that represent the overlapping subspace between the pre-training and fine tuning MDPs.   
Using fully offline pre-trained Dreamer agents we evaluated freezing and reinitialization of different combinations of submodules. 
We focused our weight \textit{freezing} experiments on the key components of the dynamics learning framework: (1) the observation encoder, (2) the recurrent model, (3) the transition prediction model, and (4) the observation prediction model. 
We focused our weight \textit{resetting} experiments on the components of the behavior learning framework: (1) the actor model, (2) the critic model, (3) the transition prediction model, and (4) the discount prediction model. 
The reward prediction model is never frozen or reset because pre-training data was gathered with a sparse reward, while fine tuning used a shaped reward.


\subsection{Data for Pretraining}

Data selection and augmentation have been shown to have a large impact on the tractability of pre-training~\cite{laskin2020reinforcement,laskin2020curl}. 
One challenge of offline-to-online reinforcement learning in general, but especially in the case of learning from expert demonstration data, is the lack of diversity afforded by exploration~\cite{levine2020offline,nair2021awac} (for a deeper discussion of the importance of diversity in exploration for all transfer learning see Chapter~\ref{chapt:transx}). 
This is the reason many popular offline reinforcement learning benchmark datasets like Atari100k and D4RL are collected from an online reinforcement \textit{learning process}, not only an expert demonstration. 
However, it is not always the case that someone would have sufficient access to an environment to train interactively.
As such, to complement the expert demonstration data we collected a simple random policy dataset in our target environments in Robosuite. 
In our experiments, we study the importance of mixing this random data in with the expert data.

For data augmentation, we were primarily interested in what approaches would best regularize the world model and policy to not overfit to the pre-training tasks, as we knew from prior work that this is an issue for both Dreamer and offline reinforcement learning.  
During training, we built on the exploration of the APT~\cite{stooke2021decoupling,wolczyk24finetuning} work and experimented with random cropping and random translation to prevent overfitting. 
For random cropping and translation, we looked at shift sizes of 2 and 4 pixels of the standard sized 64x64x3 Dreamer visual inputs.  
While we considered frame stacking and temporal augmentations such as temporal masking, prior work has shown that, especially in models using recurrent architectures, random augmentations to the temporal flow of information yields inconsistent results across tasks and environments~\cite{laskin2020curl,stooke2021decoupling}. 


% For each component, we tested three conditions: full transfer of pre-trained weights, selective reset of weights while maintaining other modules fixed, and complete freezing of the pre-trained weights during fine-tuning. 
% This factorial design resulted in $2^5 = 32$ distinct transfer configurations, enabling comprehensive analysis of cross-module dependencies and their impact on adaptation performance.

% \sum_{\tau \geq t}^{H} \hat{\gamma}^{\tau-t} \hat{r}_\tau


\section{Experiments}
\label{sec:pretraining:experiments}

In this section we provide the details of our experimental setup and review the results of the experiments.

\section{Experiment Setup}


For all experiments, we use a ``bottlenecked'' version of DreamerV3 that we call BWM, in reference to the work on concept bottlenecks in Chapter~\ref{chapt:cbwm}. 
As discussed in more detail in Chapter~\ref{chapt:cbwm}, the BWM model is nearly identical to the original DreamerV3 architecture; the only difference is that the loss-free CEM module acts as a linear transformation of the embedded state before being used by the actor, critic, or prediction modules, and performs comparably to DreamerV3. 
We use a custom "manipulation" layer configuration based on the recommended model sizes from Dreamer and the prior work on pre-training, where all MLPs had 3 layers of 640 weights.  
Beyond these changes and the investigated variations to weight freezing and resetting, all other hyperparameters are the same as the original DreamerV3 implementation to ensure consistent and reproducible training conditions. 

Our experiments are conducted with the LIBERO~\cite{liu2024libero} dataset and the Robosuite~\cite{robosuite2020} environment.
Robosuite is a realistic environment for vision-based robot manipulation, LIBERO is a dataset collected from humans that provides expert demonstrations of ``pick-and-place'' tasks, and both are motivated as tools to help transfer robot policies from simulation to the real world~\cite{zhao2020sim}. 
We were additionally motivated to study this combination of dataset and environment because while the imitation learning solutions from the LIBERO effort produced successful policies, none of the RL baselines presented in the original Robosuite effort could fully solve the pick-and-place tasks.
As such, vision-based pick-and-place manipulation tasks are a problem where the performance improvement from pre-training may be necessary for learning strong RL policies.

We utilize 64x64x3 resolution images as is standard in training Dreamer models. 
To ensure all experiments were trained with diverse of expert data all models are pre-trained on the LIBERO\_90 dataset, which has offline RL data for 50 expert demonstrations of at least 120 frames for 90 unique pick-and-place tasks.
We split the data sets into a 95\%-5\% split for validation and training, where we validate four times per epoch. 
This same split was used when pre-training uses our random behavior dataset. 
Pre-training lasts for 5 epochs of offline model-based RL. 
For our data augmentation experiments we padded these images with ``reflection padding,'' and then randomly cropped the image back down to 64x64. 
Each model is fine-tuned with online model-based RL in the Robosuite environment for an additional 500,000 environment steps, allowing for a thorough adaptation to the online setting. 
The models are fine tuned on multiple different Robosuite tasks that aims to assess how well pre-trained representations transfer to new tasks within Robosuite generally, capturing the impact of pre-training in boosting performance on the target domain.
As a baseline, DreamerV3 is also trained tabula rasa for all of tasks.

